Selective Visual Representations Improve Convergence and Generalization for Embodied AI

Embodied AI models often employ off the shelf vision backbones like CLIP to encode their visual observations. Although such general purpose representations encode rich syntactic and semantic information about the scene, much of this information is often irrelevant to the specific task at hand. This introduces noise within the learning process and distracts the agent's focus from task-relevant visual cues. Inspired by selective attention in humans-the process through which people filter their perception based on their experiences, knowledge, and the task at hand-we introduce a parameter-efficient approach to filter visual stimuli for embodied AI. Our approach induces a task-conditioned bottleneck using a small learnable codebook module. This codebook is trained jointly to optimize task reward and acts as a task-conditioned selective filter over the visual observation. Our experiments showcase state-of-the-art performance for object goal navigation and object displacement across 5 benchmarks, ProcTHOR, ArchitecTHOR, RoboTHOR, AI2-iTHOR, and ManipulaTHOR. The filtered representations produced by the codebook are also able generalize better and converge faster when adapted to other simulation environments such as Habitat. Our qualitative analyses show that agents explore their environments more effectively and their representations retain task-relevant information like target object recognition while ignoring superfluous information about other objects. Code and pretrained models are available at our project website: https://embodied-codebook.github.io.

==> old/00_abstract_v1.tex <==
Learning effective and generalizable representations remains an ongoing challenge in the field of Embodied-AI. 
While visual representations extracted from vision foundation models have demonstrated their capability in encoding useful primitives, they often carry a significant amount of information that is irrelevant to specific downstream Embodied-AI tasks. Incorporating all this information into the high-level decision-making policy can introduce high frequency noise in the learning process, distracting the agent's focus from task-relevant visual cues. In this work, we introduce a straightforward yet highly effective approach to learn the visual representations for Embodied Agents. We propose to bottleneck the task-conditioned representations using a lightweight and learnable codebook module. This codebook, when jointly trained to optimize task reward, acts as a selective filter. It purposefully excludes task-irrelevant details from the high-dimensional visual representations, while keeping only the salient visual cues essential for the given task. The resulting codebook embedding encourages more efficient exploration, leading to significant performance improvements across a variety of Embodied AI tasks, including Object Navigation in four environments and Object Displacement task. Moreover, we observe that our codebook embedding can adeptly transfer to a distinct visual domain without necessitating exhaustive end-to-end fine-tuning.

==> old/01_introduction_v1.tex <==
\section{Introduction}
\label{introduction}


\hao{We need a teaser figure to show that (1) our main technical contributions are the learnable codebook, softmax, bottleneck, (2) we can improve the object navigation results in procthor/ithor/robothor/ and better results in habitat while the RNN are frozen, and (3) the contributions are also applicable to maniplathor.}
\ranjay{Actually, as I mentioned yesterday, we should make a teaser/pull figure that lays out the main intuition instead. In our case, the intuition is that we can restrict what we see based on the task at hand. I suggest two columns. In the first column you have an abstract scene that passes through a traditional encoder and outputs a vector with words floating that describe the everything you see in the abstract scene. In the second column you have a specific task described in words and you have ``our encoder'' which outputs a smaller vector with only the relevant portion of the image highlighted.}






Our perception of the environment is not a mere reflection of the sensory input but is heavily influenced by our goals and target tasks. There's a substantial body of research in cognitive psychology and neuroscience that investigates how humans filter out irrelevant sensory input when performing specific tasks. \textit{Inattentional blindness}~\citep{simons1999gorillas} posits that we only perceive the objects and details that receive focused attention. Studies in \textit{human visual search}~\citep{wolfe1994guided, treisman1980feature} investigate how humans can search for targets in a cluttered visual environment filled with other distracting items. These studies indicate that the visual system’s limited resources process information selectively rather than comprehensively processing all of the input. The principle of \textit{top-down selective attention}~\citep{desimone1995neural, buschman2007top} highlights that our processing of the sensory data is guided by internal goals rather than external stimuli (in contrast to bottom-up processing). For instance, if you're searching for a friend wearing a red coat in a crowd, you're likely to quickly ignore people not wearing red – showcasing the top-down influence on your attention. Such selective processing of the sensory input avoids unnecessary processing of unrelated information allowing us to allocate our cognitive resources more efficiently. The application of this principle in Embodied-AI can hold the promise of improving the efficiency of sensory processing resulting in a more effective goal-directed behavior.


Embodied-AI tasks such as navigation~\citep{batra2020objectnav,krantz2023navigating}, instruction following~\citep{anderson2018vision, krantz2020beyond, shridhar2020alfred}, manipulation~\citep{ehsani2021manipulathor, xiang2020sapien}, and rearrangement~\citep{batra2020rearrangement, weihs2021visual}, often necessitate goal-directed behaviors by the agent such as navigating to a specific goal or relocating target objects. Conventional frameworks usually employ general purpose visual backbones~\citep{yadav2023offline,khandelwal2022simple} or lightweight CNN models~\citep{ehsani2022object} to extract representations from visual input. These representations are then combined with goal embeddings (\eg, GPS location, target object type or images, or natural language instructions) to construct a goal-conditioned representation $E \in \mathcal{R}^{D}$, where $D$ often has dimensions as large as $1568$, capturing an abundance of details from the visual sensory input.  Subsequently, recurrent state encoder and actor-critic components are learned based on this comprehensive representation to predict actions and state-value estimations. However, this approach can cause these components to process a significant amount of task-irrelevant information, injecting high-frequency noise into the learning process, wasting model's capacity, and distracting model's focus towards less pertinent visual cues.

% \begin{figure*}[t]
%         \centering
%         % \begin{subfigure}[b]{0.9\textwidth}
%         %     \centering
%         %     \includegraphics[width=\textwidth]{photos/EmbCLIP_framework.png}
%         %     \caption[]%
%         %     {{\small \textbf{Emb-CLIP framework}. }}    
%         %     \label{fig:framework_emb_clip}
%         % \end{subfigure}

%         % \vskip\baselineskip
%         % \vspace{-3mm}
%         \includegraphics[width=\textwidth]{photos/fig1_codebook.drawio (4).png}
%             \caption[]%
%             {{\small \textbf{Teaser}.  }}    
%             \label{fig:framework_ours}


%         \caption{{Before using codebook, and after using it.}}
%         \label{fig:models}
%     \end{figure*}

In this work, inspired by studies on human selective attention, we propose a straight-forward yet highly effective approach for bottlenecking goal-conditioned representations for Embodied agents. We introduce a \textit{codebook module} into the policy model, consiting of a collection of $K$ learnable latent codes, each with a dimension of $D_c$, where $D_c \ll D$. This codebook module, taking goal-conditioned representations $E$ as input, estimates probability scores across latent codes, and produces a codebook representation $\hat{E}$ accordingly, as illustrated in Fig.~\ref{fig:framework_ours}. By co-training the codebook module with the overall policy model to optimize task rewards, each latent code becomes associated with a goal-relevant visual cue, contributing to the representation according to its probability score. Given the substantially smaller dimension of the latent code's hidden dimension ($D_c$) compared to the original goal-conditioned embedding's dimension $D$, the codebook module acts as a selective filter, encoding only the essential cues necessary for solving the downstream task. Fig.~\ref{NN} illustrates the nearest neighbor visual observations across different latent codes, showcasing the codebook module's ability to learn essential visual cues, thereby benefit our policy. % \ainaz{Here we can point to the nearest neighbor visualizations or the probing experiments to show what kind of information is encoded in the codebook}


We demonstrate the effectiveness of our approach by achieving zero-shot, state-of-the-art performances on $2$ Embodied-AI tasks: Object Goal Navigation(ObjNav)~\citep{deitke2020robothor} and Object Displacement (ObjDis)~\citep{ehsani2022object} across $5$ benchmarks (ProcTHOR\citep{deitke2022procthor}, ArchitecTHOR, RoboTHOR~\citep{deitke2020robothor}, AI2-iTHOR\citep{ai2thor}, and ManipulaTHOR~\citep{ehsani2021manipulathor}), detailed in Sec.~\ref{sec:main_results}. For ObjNav, we pretrain the models on the ProcTHOR dataset and evaluate 0-shot on other benchmarks; for ObjDis, we follow~\citep{ehsani2022object} to train and evaluate the models in AI2-iTHOR. Across all benchmarks, our approach yields significant absolute improvements in Success Rate (SR) and Episode Length (EL).  Moreover, we further show the adaptability of our codebook representations to new visual domains by lightweight finetuning in Habitat environments~\citep{Savva_2019_ICCV} (Section.~\ref{sec:generalizability}). We intentionally design a lightweight finetuning experiment, with the majority of high-level decision-making components, including recurrent state encoder and actor-critic, remanining frozen. The focus during this lightweight finetuning is solely on adapting the goal encoder and a few CNN layers prior to the codebook module, as illustrated in \hao{Fig.?}.\ainaz{A figure showing the habitat finetuning experiment} This experiment verifies that our codebook representations can adapt to distinct visual domains in a lightweight manner.
% , efficiently capturing the essential visual cues necessary for solving the task at hand.


Finally, we conduct a comprehensive analysis, both quantitative and qualitative, to understand the factors behind the improvements. This investigation involves a thorough analysis of the visual cues encoded within our codebook representations and the consequent impact on the agent's behavior, as detailed in Sec.~\ref{sec:probing}. Our findings confirm that the codebook representations effectively keep essential visual cues while filtering out redundant details. Furthermore, we observe noticeable improvements in the agent's behavior in the form of smoother trajectories and more efficient exploration strategies.

% Our findings confirm that the codebook representations effectively retain task-critical information while filtering out extraneous environmental details. Additionally, our examinations reveal noticeable enhancements in the agent's behavior, as demonstrated in Table/Figure ? \ainaz{Top-down view of the trajectories, metric for measuring the smoothness of the paths}. These improvements manifest in the form of smoother trajectories and more efficient exploration strategies.




% Top-down selective attention~\citep{johnston1986selective, duncan1984selective, van2003selective}, is the process of prioritizing relevant sensory input while filtering out irrelevant information when having a specific goal/task at hand. Humans show remarkable skill for allocating their attention to useful sensory information when performing different tasks such as engaging in a conversation in noisy environments~\citep{broadbent2013perception}, driving, looking for a specific object in a cluttered space~\citep{rizzolatti1994space}, or navigating in a crowded scene. Broadbent's filter model of attention~\citep{broadbent2013perception}, a seminal theory in cognitive psychology, posits that a selective filter in our cognitive system acts as a bottleneck, permitting only certain stimuli to pass through for further processing while discarding irrelevant stimuli. Such a mechanism avoids unnecessary processing of unrelated information and results in a more efficient processing of relevant stimuli. 



==> old/02_related_work_v1.tex <==
\section{Related Work}

\textbf{Representation Learning for Embodied Agent.} There are various works focusing on learning performant representation for downstream Embodied AI tasks. 

\textit{Jointly learn on on-policy data:} These approach ~\citep{du2021curious,singh2022general,guo2018neural,laskin2020curl,majumdar2022ssl} learn representations for policies through contrastive learning, simultaneously optimizing task reward. In addition, many works leverage auxiliary tasks, including predicting depth~\citep{mirowski2016learning,gordon2019splitnet}, reward~\citep{jaderberg2016reinforcement}, and forward prediction~\citep{gregor2019shaping,zeng2022moving,zeng2021pushing,guo2020bootstrap}, along with inverse dynamics~\citep{pathak2017curiosity,ye2021auxiliary,ye2021auxiliaryICCV}, to enrich the learned representations. These works learn visual representation through gameplay~\citep{weihs2019learning}, dynamic graph construction~\citep{gadre2022continuous,du2020learning,savinov2018semi,wu2019bayesian} or building map representations~\citep{chaplot2020object,chaplot2020learning} on-the-fly,  In contrast, our proposed codebook module is jointly trained with the overall policy to optimize the task rewards only.

\textit{Pretrain on off-policy data:} Alternately, these methods~\citep{yadav2023offline,yadav2023ovrl,kotar2023entl,mezghan2022memory} pretrain the visual backbone or state encoder utilizing various self-supervised objectives on off-policy data collected from environments. ~\citep{wallingford2023neural,marza2023autonerf} learn 3D representations to improve agent's capacity on downstream tasks.
The EmbCLIP~\citep{khandelwal2022simple}, which leverages the large-scale, pretrained representations by CLIP~\citep{radford2021learning}, has demonstrated great promise in solving downstream EAI tasks. Our model builds upon the foundation by EmbCLIP, incorporating the proposed codebook module designed to filter out redundancies which are not essential for solving the task at hand.


\textbf{Bottleneck and regularize representation.} There have been various research progresses focus on learning representations by bottlenecking information or applying regularization, spanning fields from general machine learning~\citep{hinton2011transforming,kingma2013auto,alemi2016deep,koh2020concept,federici2020learning,mairal2008supervised}, computer vision~\citep{he2016deep,srinivas2021bottleneck,riquelme2021scaling,van2017neural,chen2023revisiting,kolesnikov2022uvim}, natural language processing~\citep{shazeer2017outrageously,fedus2022switch,mahabadi2021variational}, to reinforcement learning~\citep{serban2020bottleneck,fan2022dribo,pacelli2020learning}. Nonetheless, relatively few have implemented these techniques to the field of Embodied AI. Studies such as those by~\citep{goyal2019infobot,igl2019generalization,bai2021dynamic,lu2020dynamics} have explored learning policies incorporating information bottlenecks in fully-observed environments, such as MiniGrid~\citep{MinigridMiniworld23} or Atari~\citep{bellemare2013arcade}. In contrast, our approach is evaluated within the partially-observed, physics-enabled, and visually rich Embodied AI environments. ~\citep{kotar2023entl} develop a predictive model leveraging VQ-GAN~\citep{esser2021taming}, and ~\citep{wallingford2023neural} learn Nerf Codebooks of the environments for downstream tasks. In contrast, we learn our codebook representations jointly with policy optimization through on-policy rollout. Our codebook module design is inspired from ~\citep{han2020memory}, however, we focus on applying the learned codebook representations on the Embodied AI tasks.

==> old/03_method_v1.tex <==
\section{Methodology}

Our codebook module design is inspired from prior work~\citep{han2020memory}, however, we focus on applying the learned codebook representations on the Embodied AI tasks.

\input{Figs/framework}

We first overview the foundation policy model used for Embodied AI tasks and further introduce our contributions to make the model explore the environment more effectively in Sec.~\ref{Sec:MO}. We then present the details of our goal-conditioned cokebook representation in Sec.~\ref{Sec:CB}. Finally, we describe our training strategy in Sec.~\ref{Sec:TS}.

\subsection{Model Overview}
\label{Sec:MO}

\textbf{Preliminary.} The traditional policy models~\citep{batra2020objectnav,khandelwal2022simple} for constructing Embodied-AI agents usually share a similar core architecture. This encompasses a visual encoder that translates visual observations (\eg, RGB or depth) into a visual representation $v$; a goal encoder that encodes the task goal (\eg, GPS location, target object type, or natural language instructions) into a goal embedding $g$; and a previous action embedder to embed the most recently executed action into an action embedding $\alpha$. In this work, our model is designed to mainly\footnote{For Object Displacement task, we follow~\citep{ehsani2022object} to also include the depth sensor, the segmentation mask sensor, and the end-effector sensor.} utilize the RGB sensors for visual observations and the target object type as the task goal. Subsequent to these processes, the visual representation $v$, goal embedding $g$, and action embedding $\alpha$ are flattened and then concatenated to form the goal-conditioned observation embedding $E$. In order to derive the state estimation, a recurrent state encoder is employed to summarize the embedding over a span of time, represented as $E_t|t=1, ..., T$, resulting in the state representation $r$. Finally, the policy incorporates actor/critic heads to predict a distribution over action space as well as an estimation of the current state's value from the state representation.

% \input{Figs/codebook_module}
\textbf{Codebook module.} Our primary objective is to encourage the agent to construct a compact embedding. This enables the agent to concentrate on essential visual cues, fostering more effective exploration. To realize this, our core technical contribution lies in compressing the goal-conditioned embedding, $E \in \mathcal{R}^{D}$, where $D$ is usually large (\eg, $1568$ used in EmbCLIP). We introduce a lightweight and learnable codebook module without introducing significantly more model parameters, illustrated in Fig.~\ref{fig:models}. Specifically, the module takes the goal-conditioned embedding $E$ as input to produce a condensed goal-conditioned codebook embedding $\hat{E}$. As the training progresses, we expect that the learnable codes within the codebook module will encode a wide range of goal-conditioned visual cues, serving the agent to solve the given task. By design, we place the codebook module immediately before the recurrent state encoder. In this way, the module focuses on single-step processing, prompting the codebook to compile information at each individual step rather than relying on historical memory. On the other hand, by positioning the codebook module right after the CNN, which is in charge of fusing the visual representation $v$ with the goal embedding $g$, we ensure that the resulting representation $\hat{E}$ is goal-dependent. \hao{make sure if we have these ablation studies. otherwise, we need to remove the last sentence.} We compare our design choice with both the recurrent-codebook and visual-codebook in Sec.~\ref{sec:ablations}.

% This approach, depicted in Fig.~\ref{fig:framework_ours} effectively filters out the irrelevant sensory information for the downstream task while passing the useful information to the memory and higher levels of processing.

% \subsection{Goal-Conditioned Representations}

% \hao{We might want to merge this subsection to the model overview.}

% Embodied-AI models typically share a similar core architecture where the visual observations are encoded using a combination of pre-trained visual backbones and convolutional layers. The resulting representation is flattened by a fully connected layer and concatenated with the embeddings of other sensory input (such as GPS localization) to form the observation embedding $\mathcal{V}$. The final goal-conditioned representation $V^{\prime}$ is obtained by concatenating $\mathcal{V}$ to the goal embedding $\mathcal{G}$. $V^{\prime}$ is passed to a recurrent neural network and afterwards actor/critic heads to produce a distribution over the agent's actions. 


\subsection{goal-conditioned Codebook Embedding}
\label{Sec:CB}

In this work, we propose to compress the goal-conditioned embedding $E$ using a lightweight and learnable codebook module. The goal is to encourage the agent, based on the produced embedding $\hat{E}$, to focus on essential visual cues and foster more effective exploration. The codebook module consists of a scoring function, a collection of learnable codes, and an upsampling layer. More specifically, the module takes the goal-conditioned embedding $E$ as input, predicts probability scores for each latent codes within the codebook, applies the convex combination of the codes accordingly to construct a compact hidden embedding $h$, and then output the condensed goal-conditioned codebook embedding $\hat{E}$ after upsampling of the hidden embedding $h$. This mechanism allows the codebook module to select essential latent codes from the codebook to solve the given task, effectively filtering out redundant information from the original embedding $E$.

The codebook is defined as a latent embedding space $C = [c_1, c_2, ..., c_k] \in \mathcal{R}^{K \times D_c}$ where $K$ denotes codebook's size and $D_c$ represents the dimensionality of each latent code $c_k$. It is worth noting that, to encourage the codebook to encode the most useful cues for solving the given task, we set $D_c = 10$, which is much less than $D$. These codes are initialized randomly following a normal distribution and optimized along with the overall policy through the task objective. To extract the goal-conditioned codebook embedding $\hat{E}$ from the codebook, we first employ a scoring function $\phi(.)$ which produces a probability distribution $\mathcal{P}=\phi(E)$ over all latent codes, where $\mathcal{P} = [p_i]_{i=1}^K$ with the constraint that $\sum\mathcal{P}=1$. The scoring function $\phi$ is implemented as a single-layer MLP followed by a softmax function. This configuration aims to motivate the codebook module to select useful latent codes for addressing the given task. Subsequently, the hidden embedding $h$ is derived by taking a convex combination of the learnable codes $\{c_i\}_{i=1}^K$ in line with their associated probability scores $\mathcal{P}$:

%Instead of directly passing the goal-conditioned embedding $E$ to the following recurrent net, the embeddings are used to index the codebook $\mathcal{C}$ using an attention mechanism. An scoring function $\phi(.)$ implemented as a single-layer MLP followed by a softmax operation projects the embedding $E$ to a probability distribution $\mathcal{P}=[p_i]_{i=1}^K$ over the codebook entries (Eq.~\ref{eq:codebook_indexing}). The compressed representation $E \in \mathcal{R}^D$ is obtained by a convex combination of the learnable codes $\{c_i\}_{i=1}^K$ using the probabilities $\mathcal{P}$ (Eq.~\ref{eq:convex_combination}). 

%\begin{equation}
%    \mathcal{P} = \phi(V)
%    \label{eq:codebook_indexing}
%\end{equation}

\begin{equation}
    h = \mathcal{P}^T  C = \sum_{i=1}^{K} p_i.c_i.
    \label{eq:convex_combination}
\end{equation}
Further, the upsampling layer, implemented by a linear layer, upsamples the hidden embedding $h$ to the goal-conditioned codebook embedding $\hat{E}$. By optimizing the codebook along with the overall policy through the task objective, we expect each latent codes to associate with visual cues relevant to the task in focus. Thus, the scoring function's main job becomes recognizing and selecting necessary latent codes for solving the given task.

% When training the codebook through the task objective, we expect that each of the $K$ codebook entries will be associated with a relevant (semantic/geometric/...) primitive for the task at hand. The attention weights will indicate the extent to which each individual code contributes to the representation at time step t.

\subsection{Training Strategy}
\label{Sec:TS}

We employ Proximal Policy Optimization (PPO)~\citep{schulman2017proximal}\footnote{We follow~\citep{ehsani2022object} to use DD-PPO to optimize the policy for object displacement tasks.} to perform on-policy reinforcement learning to optimize our entire policy, including the codebook module. One critical challenge we encounter when training such codebooks is the \textit{Codebook collapse}~\citep{van2017neural,riquelme2021scaling,shazeer2017outrageously}, where only a tiny fraction of the codes are used throughout the entire training session, limiting the model's full capacity. While several solutions\footnote{We have also tried Linde-Buzo-Gray~\citep{linde1980algorithm} splitting algorithm and Gumbel Softmax~\citep{jang2016categorical} with careful temperture tunning, but have found that the dropout is the most effective approach.} have been proposed to this problem, we find that using dropout~\citep{srivastava2014dropout} is a straightforward, yet highly effective, approach to overcome it. Hence, instead of directly employing the probability scores $\mathcal{P}$ shown in the Equ.~\ref{eq:convex_combination}, we first apply dropout on it with a rate of $0.1$. It produces a new probability scores $\hat{\mathcal{P}}$, which we then use to combine the latent codes: $h = \hat{\mathcal{P}}^T  C$. Intuitively, this equates to randomly setting $10\%$ of the latent codes to zero before integrating them through a convex combination.




==> sections/_01_math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/codebook_ablations.tex <==
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{12pt}
\begin{table}[t]
		\centering
		\resizebox{\linewidth}{!}{%
		\begin{tabular}{lllllll}
			\hline
  
                \multicolumn{1}{c}{} &
                \multicolumn{1}{c}{} &
                \multicolumn{1}{c}{} &
			\multicolumn{3}{c}{\textit{Object Navigation}} 

			\\ 
% 			\cline{3-9}
                \multicolumn{1}{c}{Codebook Indexing} &
                \multicolumn{1}{c}{Codebook Size} &
                \multicolumn{1}{c}{Goal-Conditioned} &
            \multicolumn{1}{c}{\textbf{SR(\%)}$\uparrow$} &
            \multicolumn{1}{c}{\textbf{EL}$\downarrow$}  &
			\multicolumn{1}{c}{\textbf{SPL}$\uparrow$} \\
			
			\hline
			
			\multicolumn{1}{l}{} &
                \multicolumn{1}{c}{1024 \times 10} &
                \multicolumn{1}{c}{\cmark} &
			\multicolumn{1}{c}{72.56} &
                \multicolumn{1}{c}{119} &
			\multicolumn{1}{c}{48.88}  \\

			\multicolumn{1}{l}{Softmax} &
                \multicolumn{1}{c}{256 \times 10} &
                \multicolumn{1}{c}{\cmark} &
			\multicolumn{1}{c}{\textbf{73.4}} &
                \multicolumn{1}{c}{124} &
			\multicolumn{1}{c}{\textbf{49.84}}  \\

			\multicolumn{1}{l}{} &
                \multicolumn{1}{c}{256 \times 10} &
                \multicolumn{1}{c}{\xmark} &
			\multicolumn{1}{c}{65.31} &
                \multicolumn{1}{c}{134} &
			\multicolumn{1}{c}{43.62}  \\

                % \cline{2-7}

			\multicolumn{1}{l}{Top-1 gating} &
                \multicolumn{1}{l}{} &
                \multicolumn{1}{c}{} &
			\multicolumn{1}{c}{38.06} &
                \multicolumn{1}{c}{\textbf{110}} &
			\multicolumn{1}{c}{29.39}  \\

			\multicolumn{1}{l}{Top-8 gating} &
                \multicolumn{1}{c}{256 \times 10} &
                \multicolumn{1}{c}{\cmark} &
			\multicolumn{1}{c}{68.22} &
                \multicolumn{1}{c}{160} &
			\multicolumn{1}{c}{45.86}  \\


			\multicolumn{1}{l}{Top-32 gating} &
                \multicolumn{1}{l}{} &
                \multicolumn{1}{c}{} &
			\multicolumn{1}{c}{73.27} &
                \multicolumn{1}{c}{138} &
			\multicolumn{1}{c}{48.5}  \\

                % \cline{2-7}

			\multicolumn{1}{l}{EmbCLIP Baseline} &
                \multicolumn{1}{c}{-} &
                \multicolumn{1}{c}{-} &
			\multicolumn{1}{c}{59.81} &
                \multicolumn{1}{c}{176} &
			\multicolumn{1}{c}{43.91}  \\



                \hline


		\end{tabular}%
		}
		\vspace{2mm}
		\captionof{table}{\footnotesize{\textbf{ Ablations of the Codebook.} 
		}}\label{table:ablation_results}
    \addtolength{\tabcolsep}{4pt} 
    \vspace{-4mm}
\end{table}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}

==> tables/linear_probing.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{15pt}
\begin{table}[t]
		\centering
		\resizebox{0.8\linewidth}{!}{%
    		\begin{tabular}{llll}
    
    % 			\cline{3-9}
    \hline
    			\multicolumn{1}{c}{Task} & 
                    \multicolumn{1}{c}{Model} &
                    \multicolumn{1}{c}{\textbf{Accuracy}$\uparrow$} &
                    \multicolumn{1}{c}{\textbf{F1 Score}$\uparrow$} \\    			
    			\hline
    


        \hline
    
                    \multicolumn{1}{l}{Object Presence } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{\textbf{0.10}}&
    			\multicolumn{1}{r}{\textbf{0.55}} \\
    		
    
    
                    \multicolumn{1}{c}{(all 125 categories)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{0.05}&
    			\multicolumn{1}{r}{0.29} \\
    
       \hline
    
                    \multicolumn{1}{l}{Object Presence } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{\textbf{0.36}}&
    			\multicolumn{1}{r}{\textbf{0.53}} \\
    		
    
    
                    \multicolumn{1}{c}{(16 goal categories)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{0.27}&
    			\multicolumn{1}{r}{0.11} \\
    
    
    
    
       \hline
    
    
                    \multicolumn{1}{l}{Goal Visibility } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{0.87} &
    			\multicolumn{1}{r}{-} \\
    			
    
    
                    \multicolumn{1}{l}{(binary)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{\textbf{0.92}}&
    			\multicolumn{1}{r}{-} \\


       \hline
    
    
                    \multicolumn{1}{l}{Distance to Goal } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{0.29} &
    			\multicolumn{1}{r}{-}\\
    			
    
    
                    \multicolumn{1}{c}{(5-way classification)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{\textbf{0.31}} &
    			\multicolumn{1}{r}{-} \\
    
    
    
    
       % \hline
    
    
       %              \multicolumn{1}{c}{} &
    			% \multicolumn{1}{l}{EmbCLIP} &
       %              \multicolumn{1}{l}{before RNN} &
    			% \multicolumn{1}{c}{} \\
    			
       %              \multicolumn{1}{c}{Obstacle in Front} &
    			% \multicolumn{1}{l}{} &
       %              \multicolumn{1}{l}{after RNN} &
    			% \multicolumn{1}{c}{} \\    
       %              \cline{3-4}
    
       %              \multicolumn{1}{c}{} &
    			% \multicolumn{1}{l}{EmbCLIP-Codebook } &
       %              \multicolumn{1}{l}{before RNN} &
    			% \multicolumn{1}{c}{} \\
    
       %              \multicolumn{1}{c}{} &
    			% \multicolumn{1}{l}{} &
       %              \multicolumn{1}{l}{after RNN} &
    			% \multicolumn{1}{c}{} \\
    
    
    
       % \hline
    
    			
       %              \multicolumn{1}{c}{Visited Room (binary)} &
    			% \multicolumn{1}{l}{EmbCLIP} &
    			% \multicolumn{1}{c}{0.63} &
    			% \multicolumn{1}{c}{-} \\   
    
       %              \multicolumn{1}{c}{} &
    			% \multicolumn{1}{l}{EmbCLIP-Codebook } &
    			% \multicolumn{1}{c}{\textbf{0.68}} &
    			% \multicolumn{1}{c}{-}\\
    
       % \hline
    
    			
       %              \multicolumn{1}{c}{Visited Position} &
    			% \multicolumn{1}{l}{EmbCLIP} &
       %              \multicolumn{1}{l}{after RNN} &
    			% \multicolumn{1}{c}{0.76} \\
    
       %              \multicolumn{1}{c}{} &
    			% \multicolumn{1}{l}{EmbCLIP-Codebook } &
       %              \multicolumn{1}{l}{after RNN} &
    			% \multicolumn{1}{c}{\textbf{0.78}} \\
    		\end{tabular}%
		}
		\vspace{2mm}
		\captionof{table}{\footnotesize{\textbf{ Results for models trained on ProcTHOR and evaluated 0-shot on several Object Goal Navigation benchmarks. \ani{Needs updating}} 
		}}\label{table:probing}
    % \addtolength{\tabcolsep}{4pt} 
    \vspace{-4mm}
\end{table}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}



==> tables/linear_probing_codebook_ablations.tex <==
\begin{table}[t]
\begin{minipage}{.4\linewidth}
  \centering
  \caption{{\small Linear probing shows codebook embeddings encode more task-relevant cues}}
  \vspace{-2mm}
  \tiny
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.2}
    		\begin{tabular}{llll}
    
    % 			\cline{3-9}
    \hline
    			\multicolumn{1}{c}{Task} & 
                    \multicolumn{1}{c}{Model} &
                    \multicolumn{1}{c}{\textbf{Accuracy}$\uparrow$} &
                    \multicolumn{1}{c}{\textbf{F1 Score}$\uparrow$} \\    			
    			\hline
    


        \hline
    
                    \multicolumn{1}{l}{Object Presence } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{\textbf{0.10}}&
    			\multicolumn{1}{r}{\textbf{0.55}} \\
    		
    
    
                    \multicolumn{1}{l}{(all 125 categories)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{0.05}&
    			\multicolumn{1}{r}{0.29} \\
    
       \hline
    
                    \multicolumn{1}{l}{Object Presence } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{\textbf{0.36}}&
    			\multicolumn{1}{r}{\textbf{0.53}} \\
    		
    
    
                    \multicolumn{1}{l}{(16 goal categories)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{0.27}&
    			\multicolumn{1}{r}{0.11} \\
    
    
    
    
       \hline
    
    
                    \multicolumn{1}{l}{Goal Visibility } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{0.87} &
    			\multicolumn{1}{r}{-} \\
    			
    
    
                    \multicolumn{1}{l}{(binary)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{\textbf{0.92}}&
    			\multicolumn{1}{r}{-} \\


       \hline
    
    
                    \multicolumn{1}{l}{Distance to Goal } &
    			\multicolumn{1}{l}{EmbCLIP} &
    			\multicolumn{1}{r}{0.29} &
    			\multicolumn{1}{r}{-}\\
    			
    
    
                    \multicolumn{1}{c}{(5-way classification)} &
    			\multicolumn{1}{l}{+Codebook } &
    			\multicolumn{1}{r}{\textbf{0.31}} &
    			\multicolumn{1}{r}{-} \\
       \hline
    
    		\end{tabular}%
\label{table:probing}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.5\linewidth}
  \centering
  \caption{{\small Ablations of Different Codebook Hyper-Parameters on ProcTHOR-10k (test) Object Navigation.}} 
  \vspace{-2mm}
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.1}
		\begin{tabular}{lllllll}
			\hline
  
                \multicolumn{1}{c}{} &
                \multicolumn{1}{c}{} &
                \multicolumn{1}{c}{Goal-} &
			\multicolumn{3}{c}{\textit{Object Navigation}} 

			\\ 
% 			\cline{3-9}
                \multicolumn{1}{c}{Codebook Indexing} &
                \multicolumn{1}{c}{Codebook Size} &
                \multicolumn{1}{c}{Conditioned} &
            \multicolumn{1}{c}{\textbf{SR(\%)}$\uparrow$} &
            \multicolumn{1}{c}{\textbf{EL}$\downarrow$}  &
			\multicolumn{1}{c}{\textbf{SPL}$\uparrow$} \\
			
			\hline
			
			\multicolumn{1}{l}{} &
                \multicolumn{1}{c}{1024 $\times$ 10} &
                \multicolumn{1}{c}{\cmark} &
			\multicolumn{1}{c}{72.56} &
                \multicolumn{1}{c}{119} &
			\multicolumn{1}{c}{48.88}  \\

			\multicolumn{1}{l}{Softmax} &
                \multicolumn{1}{c}{256 $\times$ 10} &
                \multicolumn{1}{c}{\cmark} &
			\multicolumn{1}{c}{\textbf{73.4}} &
                \multicolumn{1}{c}{124} &
			\multicolumn{1}{c}{\textbf{49.84}}  \\

			\multicolumn{1}{l}{} &
                \multicolumn{1}{c}{256 $\times$ 10} &
                \multicolumn{1}{c}{\xmark} &
			\multicolumn{1}{c}{65.31} &
                \multicolumn{1}{c}{134} &
			\multicolumn{1}{c}{43.62}  \\

                \hline

			\multicolumn{1}{l}{Top-1 gating} &
                \multicolumn{1}{l}{} &
                \multicolumn{1}{c}{} &
			\multicolumn{1}{c}{38.06} &
                \multicolumn{1}{c}{\textbf{110}} &
			\multicolumn{1}{c}{29.39}  \\

			\multicolumn{1}{l}{Top-8 gating} &
                \multicolumn{1}{c}{256 $\times$ 10} &
                \multicolumn{1}{c}{\cmark} &
			\multicolumn{1}{c}{68.22} &
                \multicolumn{1}{c}{160} &
			\multicolumn{1}{c}{45.86}  \\


			\multicolumn{1}{l}{Top-32 gating} &
                \multicolumn{1}{l}{} &
                \multicolumn{1}{c}{} &
			\multicolumn{1}{c}{73.27} &
                \multicolumn{1}{c}{138} &
			\multicolumn{1}{c}{48.5}  \\

                \hline

			\multicolumn{1}{l}{EmbCLIP Baseline} &
                \multicolumn{1}{c}{-} &
                \multicolumn{1}{c}{-} &
			\multicolumn{1}{c}{59.81} &
                \multicolumn{1}{c}{176} &
			\multicolumn{1}{c}{43.91}  \\



                \hline


		\end{tabular}%
  \label{table:ablation_results}
\end{minipage}
\vspace{-6mm}
\end{table}


==> tables/manipulathor_results.tex <==
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{10pt}
\begin{table}[t]
		\centering
		\resizebox{0.6\linewidth}{!}{
		\begin{tabular}{llll}
  \hline
			\multicolumn{1}{c}{} & 
                \multicolumn{1}{c}{} &
			\multicolumn{2}{c}{\textit{Object Displacement}} 

			\\ 
% 			\cline{3-9}
			\multicolumn{1}{c}{Benchmark} & 
                \multicolumn{1}{c}{Model} &
                \multicolumn{1}{c}{\textbf{PU(\%)}$\uparrow$} &
			\multicolumn{1}{c}{\textbf{SR(\%)}$\uparrow$}  \\
			
			\hline
			
                \multicolumn{1}{c}{ManipulaTHOR} &
			\multicolumn{1}{l}{m-VOLE} &
			\multicolumn{1}{c}{81.2} &
			\multicolumn{1}{c}{59.6}  \\

                \multicolumn{1}{c}{} &
			\multicolumn{1}{l}{m-VOLE-Codebook} &
			\multicolumn{1}{c}{\textbf{86.0}} &
			\multicolumn{1}{c}{\textbf{65.1}}  \\

    \hline

		\end{tabular}
		}
		\vspace{2mm}
		\captionof{table}{\footnotesize{\textbf{ Results of Object Displacement task.} 
		}}\label{table:OD_results}
    \addtolength{\tabcolsep}{4pt} 
    \vspace{-4mm}
\end{table}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}

==> tables/objnav_dino_results.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{10pt}
\begin{table}[t]
	\centering
 \vspace{-1mm}
 \captionof{table}{\footnotesize{Our method with the codebook consistently outperforms the baselines using DINOv2~\citep{oquab2023dinov2} visual features in zero-shot evaluation on $4$ Object Goal Navigation benchmarks. We use $\uparrow$ and $\downarrow$ to denote if larger or smaller values are preferred.}
	}
 \vspace{-2mm}
	\resizebox{0.85\linewidth}{!}{
	\begin{tabular}{lllllll}
  	\toprule
		 & 
             &
		\multicolumn{5}{c}{Object navigation} \\
            \cline{3-7}
		Benchmark & 
            Model &
            \multicolumn{1}{r}{SR(\%)$\uparrow$} &
		\multicolumn{1}{r}{EL$\downarrow$} &
		\multicolumn{1}{r}{Curvature$\downarrow$} & 
            \multicolumn{1}{r}{SPL$\uparrow$} &
            \multicolumn{1}{r}{SEL$\uparrow$} \\
		\midrule
		\multirow{2}{*}{ProcTHOR-10k (test) } &

		DINOv2~\citep{oquab2023dinov2} &
		\multicolumn{1}{r}{74.25} &
		\multicolumn{1}{r}{151.00}  &
		\multicolumn{1}{r}{0.24} & 
            \multicolumn{1}{r}{49.53} &
            \multicolumn{1}{r}{43.20} \\
		&
		+Codebook (Ours) &
		\multicolumn{1}{r}{\textbf{76.31}} &
		\multicolumn{1}{r}{\textbf{129.00}} &
		\multicolumn{1}{r}{\textbf{0.12}} & 
            \multicolumn{1}{r}{\textbf{50.26}} &
            \multicolumn{1}{r}{\textbf{44.70}} \\
            
		\midrule
		\multirow{2}{*}{\textsc{Architec}THOR (0-shot)} &
		
		DINOv2 &
		\multicolumn{1}{r}{57.25} &
		\multicolumn{1}{r}{218.00}  &
		\multicolumn{1}{r}{0.25} & 
            \multicolumn{1}{r}{36.83} &
            \multicolumn{1}{r}{29.00} \\
		&
		+Codebook (Ours) &
		\multicolumn{1}{r}{\textbf{59.75}} &
		\multicolumn{1}{r}{\textbf{194.00}} &
		\multicolumn{1}{r}{\textbf{0.11}} & 
            \multicolumn{1}{r}{\textbf{36.00}} &
            \multicolumn{1}{r}{\textbf{31.70}} \\
            
		\midrule
  
		\multirow{2}{*}{AI2-iTHOR (0-shot)} &
		DINOv2 &
		\multicolumn{1}{r}{74.67} &
		\multicolumn{1}{r}{97.00}  &
		\multicolumn{1}{r}{0.19} & 
            \multicolumn{1}{r}{59.45} &
            \multicolumn{1}{r}{26.50} \\
		&
		+Codebook (Ours) &
		\multicolumn{1}{r}{\textbf{76.93}} &
		\multicolumn{1}{r}{\textbf{68.00}} &
		\multicolumn{1}{r}{\textbf{0.07}} & 
            \multicolumn{1}{r}{\textbf{60.14}} &
            \multicolumn{1}{r}{\textbf{28.30}} \\

            \midrule

            \multirow{2}{*}{RoboTHOR (0-shot)} &
		DINOv2 &
		\multicolumn{1}{r}{60.54} &
		\multicolumn{1}{r}{-}  &
		\multicolumn{1}{r}{-} & 
            \multicolumn{1}{r}{\textbf{29.36}} &
            \multicolumn{1}{r}{-} \\
		&
		+Codebook (Ours) &
		\multicolumn{1}{r}{\textbf{61.03}} &
		\multicolumn{1}{r}{-} &
		\multicolumn{1}{r}{-} & 
            \multicolumn{1}{r}{28.01} &
            \multicolumn{1}{r}{-} \\
		
            
		\bottomrule
            
	\end{tabular}
	}
	\label{table:dino_results}
    \addtolength{\tabcolsep}{4pt} 
    \vspace{-2mm}
\end{table}


==> tables/objnav_skip_connection.tex <==


\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{14pt}
\begin{table}[t]
	\centering
 \vspace{-1mm}
 \captionof{table}{\footnotesize{\textcolor{red}{We use $\uparrow$ and $\downarrow$ to denote if larger or smaller values are preferred.}
	}}
 \vspace{-2mm}
	\resizebox{0.85\linewidth}{!}{
	\begin{tabular}{lllll}
  	\toprule
		 & 
             &
		\multicolumn{3}{c}{Object navigation} \\
            \cline{3-5}
		Benchmark & 
            Model &
            \multicolumn{1}{r}{SR(\%)$\uparrow$} &
		\multicolumn{1}{r}{EL$\downarrow$} &
            \multicolumn{1}{r}{SPL$\uparrow$} \\
		\midrule
		\multirow{3}{*}{ProcTHOR-10k (test) } &

		  EmbCLIP &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{}  &
            \multicolumn{1}{r}{} \\
            &
		EmbCLIP-Codebook &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{} &
            \multicolumn{1}{r}{} \\
		&
		EmbCLIP-Codebook + Skip Connection &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{} &
            \multicolumn{1}{r}{} \\
           
            
		\midrule
		\multirow{3}{*}{\textsc{Architec}THOR (0-shot)} &
		
		EmbCLIP &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{}  &
            \multicolumn{1}{r}{} \\
            &
		EmbCLIP-Codebook &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{} &
            \multicolumn{1}{r}{} \\
		&
		EmbCLIP-Codebook + Skip Connection &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{} &
            \multicolumn{1}{r}{} \\
            
		\midrule
  
		\multirow{3}{*}{AI2-iTHOR (0-shot)} &
		EmbCLIP &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{}  &
            \multicolumn{1}{r}{} \\
            &
		EmbCLIP-Codebook &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{} &
            \multicolumn{1}{r}{} \\
		&
		EmbCLIP-Codebook + Skip Connection &
		\multicolumn{1}{r}{} &
		\multicolumn{1}{r}{} &
            \multicolumn{1}{r}{} \\

		
            
		\bottomrule
            
	\end{tabular}
	}
	\label{table:skip_conection}
    \addtolength{\tabcolsep}{4pt} 
    \vspace{-2mm}
\end{table}

